Valence bond solid formalism for d-level one-way quantum computation

The d-level or qudit one-way quantum computer (d1WQC) is described using the valence bond solid formalism and the generalised Pauli group. This formalism provides a transparent means of deriving measurement patterns for the implementation of quantum gates in the computational model. We introduce a new universal set of qudit gates and use it to give a constructive proof of the universality of d1WQC. We characterise the set of gates that can be performed in one parallel time step in this model.

==> includes/seans-commands.tex <==
%------------------------------------------------------------------
%   Start Sean's Commands
%------------------------------------------------------------------
\newcommand{\mbf}{\mathbf}  % Tells the compiler to switch into math-style bold-face
\newcommand{\R}{\mathbb{R}} % To use the symbol for the set of real numbers, type \R
\newcommand{\N}{\mathbb{N}} % To use the symbol for the set of natural numbers type \N
\newcommand{\C}{\mathbb{C}} % To use the symbol for the set of complex numbers type \C
\newcommand{\Z}{\mathbb{Z}} % To use the symbol for the set of integers type \Z
\newcommand{\Q}{\mathbb{Q}} % To use the symbol for the set of rational numbers type \Q
\newcommand{\modp}{(\mbox{mod p})}
\newcommand{\modd}{(\mbox{mod d})}
\newcommand{\gset}[1]{\left\langle #1 \right\rangle}
\newcommand{\ket}[1]{| #1 \rangle}
\newcommand{\bra}[1]{\langle #1 |}
\newcommand{\ip}[2]{\langle #1 | #2 \rangle}
\newcommand{\zero}{\ket{0}}
\newcommand{\one}{\ket{1}}

\newcommand{\nzer}[2]{\mathcal{N}_{#1}(#2)}  % To symbolise the normaliser
\newcommand{\nzeri}[1]{\mathcal{N}(#1)}  % To symbolise the normaliser with implicit ambient group
\newcommand{\G}{\mathcal{G}}  % To symbolise mathcal G - for groups
\newcommand{\gate}[1]{\left( \begin{matrix} #1 \end{matrix} \right)}
\newcommand{\smallGate}[1]{\left( \begin{smallmatrix} #1 \end{smallmatrix} \right)}

\newcommand{\cnd}{Cl^n_d}
\newcommand{\cbd}{Cl^n_2}
\newcommand{\pnd}{\mathcal{P}^n_d}
\newcommand{\pbd}{\mathcal{P}^n_2}
\newcommand{\pauli}[2]{\mathcal{P}_{#1}^{\otimes #2}}
\newcommand{\pauliOne}[1]{\mathcal{P}_{#1}}
\newcommand{\clifford}[2]{\mathcal{C}l_{#1}^{\otimes #2}}
\newcommand{\cliffordOne}[1]{\mathcal{C}l_{#1}}

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\bes}{\begin{equation*}}
\newcommand{\ees}{\end{equation*}}
\newcommand{\beas}{\begin{eqnarray*}}
\newcommand{\eeas}{\end{eqnarray*}}

\newcommand{\dWQC}{d1WQC } %$_d$

\setcounter{tocdepth}{2}

%------------------------------------------------------------------
%   End Sean's Commands
%------------------------------------------------------------------

==> includes/section-pauli-old.tex <==
A basic ingredient in our description of the workings of the d-1WQC are the generalised Pauli groups of quantum gates.  In this section we review the Pauli group on $n$ qubits and describe the natural extension to $n$ qudits.  We also define the gates that normalise the Pauli group, the Clifford group.  In doing so we establish the notation used throughout this paper.

The Pauli group of quantum gates on one qubit, denoted $\pauliOne{2}$ are generated by

\be
\sigma_x = \smallGate{ 0 & 1 \\ 1 & 0},
\sigma_z = \smallGate{ 1 & 0 \\ 0 & -1 }
\ee

%We will also use the notation $X = \sigma_x$, $Y = \sigma_y$ and $Z = \sigma_z$.

\begin{defn}
The Pauli group is defined as $\gset{\sigma_x,\sigma_y,\sigma_z}$, i.e. the group generated by $\sigma_x$, $\sigma_y$ and $\sigma_z$.  It is a group of order 16 consisting of $(2 \times 2)$ complex valued unitary matrices i.e. a subgroup of $U(2)$.  We will denote the group generated as $\pauliOne{2}$ meaning the Pauli group on one qubit.
\end{defn}

We naturally extend the Pauli group to tensor product spaces of $n$ qubits which we denote $\pauli{2}{n}$ which is defined as

\be
\pauli{2}{n} = \left\{\bigotimes_{k=1}^{n} p_k : p_k \in \pauliOne{2} \right\}
\ee

%We can see that the order of $\pauli{2}{n}$ is $4^{n+1}$

Next we consider the Clifford group on $n$ qubits.  This is defined as being the normaliser of the Pauli group within the unitary group.
\begin{defn}

The Clifford group of operators on $n$ qubits, $\clifford{2}{n}$, is defined to be the set
of quantum gates that map the Pauli group $\pauli{2}{n}$ to itself under
conjugation.  I.e.

\be
\clifford{2}{n} = \left\{ c \in U(2^n): c p c^{\dagger} \in \pauli{2}{n}, \forall p \in \pauli{2}{n} \right\}
\ee
\end{defn}

We have some useful gates that are used throughout the paper, the two-qubit matrix controlled-NOT denoted $CNOT$
\be
 CNOT = \smallGate{ 1 & 0 & 0 & 0 \\
                                        0 & 1 & 0 & 0 \\
                                        0 & 0 & 0 & 1 \\
                                        0 & 0 & 1 & 0 }
\ee
The one-qubit Hadamard matrix
\be
H = \frac{1}{\sqrt{2}}\smallGate{ 1 & 1 \\ 1 & -1 }
\ee

The $\frac{\pi}{4}$ phase gate \be
 S = \left( \begin{smallmatrix} 1 & 0 \\
0 & i
\end{smallmatrix} \right)
\ee
Another useful two-qubit matrix is the controlled-Z or
\be
C_Z = diag(1,1,1,-1)
\ee
where $diag$ denotes a diagonal matrix with diagonal entries as specified and zeros elsewhere.

In fact $H$, $S$, $CNOT$ and $C_Z$ are all gates in the Clifford group and furthermore it was shown in \cite{gottesmanPhd} that, up to a global phase factor, $H$ and $S$ together generate  and $H$, $S$, and $CNOT$ together generate for any $n$.

In this paper we are considering models of computation that use d-level systems or qudits as the unit of subdivision for the computational space so we must define the natural generalisation of the Pauli group to systems of qudits.

Acting on d-level quantum systems where $d>2$ we define the one qudit gates $X$ and $Z$ such that for $j \in
\Z_d$ (where $\Z_d$ denotes the ring of integers modulo $d$ sometimes denoted $\Z/d\Z$)
\be
X\ket{j} = \ket{j+1\modd}
\ee
\be
Z\ket{j} = \omega^j\ket{j}
\ee
where $\omega = exp\left(\frac{2\pi i}{d}\right)$ is the $d^{th}$ root of unity.  We note the crucial relation
\be
ZX = \omega XZ
\ee

\label{defn_gen_pauli}\defn{The generalised Pauli group on one qudit, $\pauliOne{d}$, is defined as $\gset{X, Z}$ and the pauli group on $n$ qudits is defined as
\begin{equation}
\pauli{d}{n} = \left\{\bigotimes_{k=1}^{n} p_k : p_k \in \pauliOne{d} \right\}
\end{equation}
}

Note that if we used this definition for $d=2$ then we would not obtain the Pauli group as defined above.  Instead we would have the real Pauli group which is generated by $\sigma_x$ and $\sigma_z$ (this nomenclature matches that given to the real and complex Clifford groups in \cite{invariantsClifford}).  Since the real Pauli group on one qubit does not have the $S$ gate in its normaliser, we use instead the complex Pauli group in the definition on one qubit given above for $\pauliOne{2}$.  In fact when $d$ is an odd prime the unitary matrices in $\pauli{d}{n}$ form a faithful irreducible representation of an extra-special p-group of order $d^3$ \cite{rep_char_group}.  The real Pauli group on one qubit forms the natural base of this sequence.

Using the relation $ZX = \omega XZ$ we note that we can express $\pauli{d}{n}$ as
\be
\pauli{d}{n} = \left\{ \omega^kZ_1^{a_1}X_1^{b_1}...Z_n^{a_n}X_n^{b_n} : a_j,b_j,k \in \Z_d \right\}
\ee
Here the subscripts label upon which qudit the operator acts. Often we will not be interested in the the global phase $\omega^k$.  In this case we may considered the central quotient group $\pauli{d}{n} / Z(\pauli{d}{n})$ (where $Z(\pauli{d}{n})$ denotes the centre of the group) with representatives of the form $Z_1^{a_1}X_1^{b_1}...Z_n^{a_n}X_n^{b_n}$.

\begin{defn}\label{defn_gen_clifford}
The Clifford group on $n$ qudits, $\clifford{d}{n}$, is defined to be the normaliser of $\pauli{d}{n}$ in $U(d^n)$.  That is
\be
\clifford{d}{n} = \{c \in U(d^n): cpc^\dagger \in \pauli{d}{n}\mbox{ for all }
p \in \pauli{d}{n}\}
\ee
\end{defn}

We can interpret each $c \in \clifford{d}{n}$ as an endomorphism of $\pauli{d}{n}$ by which we mean its action under conjugation.  This is denoted as
\be
g \mapsto_c h\mbox{ for }g,h \in \pauli{d}{n}
\ee
whenever $cgc^\dagger = h$

Given any element $c \in \clifford{d}{n}$ and any phase factor $\alpha = exp(i\theta)$ then $\alpha c \in \clifford{d}{n}$.  It is clear that $c$ and $\alpha c$ induce the same endomorphism on $\pauli{d}{n}$.  For this reason we treat elements of $\clifford{d}{n}$ to be equivalent if they differ only by a global phase factor.

The generalisation to the qudit case of the $H$, $S$, controlled-NOT and controlled-Z gates are as follows. H becomes the quantum Fourier transform on one qudit, which we denote by $F$ where
\be
F \ket{j} = \frac{1}{\sqrt{d}}\sum_{m \in \Z_d} \omega^{jm} \ket{m}
\ee
For the case where $d$ is odd we have the definition
\be
S \ket{j} = \omega^{\frac{j}{2}(j+1)} \ket{j}
\ee
and
\be
C_X \ket{j}\ket{k} = \ket{j}\ket{j+k(\mbox{mod }d)}
\ee
\be
C_Z \ket{j} \ket{k} = \omega^{jk} \ket{j}\ket{k}
\ee
We prove in the appendix that any Clifford circuit on $n$ qudits, where $d$ is an odd prime, can be constructed up to a global phase by the gates $\set{C_X,F,S}$.
